Cosmic-ray propagation in extragalactic space and secondary messengers

These notes summarize the lectures about "Cosmic-ray propagation in extragalactic space and secondary messengers", focusing in particular on the interactions of cosmic-ray particles with the background photons in the Universe, including nuclear species heavier than hydrogen, and on the analytical computation of the expected cosmic-ray fluxes at Earth. The lectures were held at the Course 208 of the International School of Physics "Enrico Fermi" on "Foundations of Cosmic-Ray Astrophysics", in Varenna (Como, Italy) from June 23rd to June 29th, 2022. These notes are complementary to the content of the lectures held by Pasquale Dario Serpico at the same school.

==> suggestions.tex <==
\section{Description}
This is a very short sample paper distributed with the class
\texttt{cimento}.
It is just a collection of examples about the syntax of commands
which behave in a different way from the standard \LaTeX
and/or new commands not defined in \LaTeX.


%\begin{figure}
%\includegraphics{foo}     % includes figure foo.eps
%\caption{Description of the figure.}
%\end{figure}


This sample is not meant to provide the complete documentation for the class.
You can also use this file as a template for your own paper:
copy it to another filename and then modify as needed.

\section{Examples}

\subsection{Tables}
Table~\ref{tab:pricesI}
inserted at this point.

\begin{table}
  \caption{Prices of important items.}
  \label{tab:pricesI}
  \begin{tabular}{rcl}
    \hline
      Item 1      & 1500  & EUR    \\
      Item 2 & 15000 & EUR    \\
      Item 3      & 1500  & dollars \\
    \hline
      Item 4     & .25   & dollars \\
      Item 5         & 1.25  & dollars \\
      Item 6         & 1     & dollars \\
    \hline
  \end{tabular}
\end{table}





\subsection{Mathematics}
Here is a lettered array~(\ref{e.all}), with eqs.~(\ref{e.house})
and~(\ref{e.phi}):
\begin{eqnletter}
 \label{e.all}
 \drm x_\sy{F} & = & 1.2\cdot10^3\un{cm}, \qquad
                     \tx{where\ } \sy{F} = \tx{Fermi}    \label{e.house}\\
 \phi_i        & = & i\pi                                \label{e.phi}
\end{eqnletter}

\subsection{Citations}
We're almost done, just some citations~\cite{ref:apo}
and we will be over~\cite{ref:pul,ref:bra}.
 

